RWKVQuant: Quantizing the RWKV Family with Proxy Guided Hybrid of Scalar and Vector Quantization

RWKV is a modern RNN architecture with comparable performance to Transformer, but still faces challenges when deployed to resource-constrained devices. Post Training Quantization (PTQ), which is a an essential technique to reduce model size and inference latency, has been widely used in Transformer models. However, it suffers significant degradation of performance when applied to RWKV. This paper investigates and identifies two key constraints inherent in the properties of RWKV: (1) Non-linear operators hinder the parameter-fusion of both smooth- and rotation-based quantization, introducing extra computation overhead. (2) The larger amount of uniformly distributed weights poses challenges for cluster-based quantization, leading to reduced accuracy. To this end, we propose RWKVQuant, a PTQ framework tailored for RWKV models, consisting of two novel techniques: (1) a coarse-to-fine proxy capable of adaptively selecting different quantization approaches by assessing the uniformity and identifying outliers in the weights, and (2) a codebook optimization algorithm that enhances the performance of cluster-based quantization methods for element-wise multiplication in RWKV. Experiments show that RWKVQuant can quantize RWKV-6-14B into about 3-bit with less than 1% accuracy loss and 2.14x speed up.

==> tabs/quarot_extra_flops.tex <==
% 额外增加的flops
%total  2.608112 * 10e12

%quarot
%14B 35,537,260 * token
%7B  18,642,476 * token

%smooth
%14B  3,150,528 * token
%7B   1,652,736 * token

% 额外增参数量
%qurot
%14B 5,550,000
%7B  2,622,618

%smooth
%14B  3,150,528
%7B   1,652,736

rwkv  uf=1.5 uc=60
14B  58%  使用SQ
7B 60%

llama
14B  8%
7B 10%

==> texs/1_intro.tex <==
\section{Introduction}\label{sec_intro}
% 1.背景：介绍 RWKV
RWKV~\cite{peng2023rwkv} is a modern sequence model that integrates the strengths of both Recurrent Neural Networks (RNNs)~\cite{elman1990finding} and Transformer~\cite{vaswani2017attention}, particularly recognized for its exceptional performance and constant inference overhead. 
The model's design enhances two essential techniques, Attention Free Transformer (AFT)~\cite{zhai2021attention} and GeGLU~\cite{shazeer2020glu}, as replacements for the Attention mechanism of Transformer. 
RWKV further introduces a token-shift method that blends each token with its preceding one, enabling linear complexity of the inference process.
These modifications have endowed RWKV a comparable capacity to Transformer-based Large Language Models (T-LLMs) while retaining the efficient inference feature of RNNs, positioning it a promising foundational architecture for both language~\cite{peng2024eagle} and vision~\cite{zhou2024bsbp} tasks. 
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.4\textwidth]{imgs/quant_res_compare.png}
    \caption{Accuracy-model size curve. Results of zero-shot accuracy are evaluated on the LAMBADA dataset~\cite{radford2019language}. 
    % The plot compares the accuracy versus model size in MB for RWKV models on the LAMBADA dataset. The FP16 curve represents the baseline before quantization, while Hybrid-3.2bit, SQ-GPTQ-3.5bit, and VQ-GPTVQ-3.5bit show results after applying respective quantization methods.
    }
    \vspace{-4mm}
    \label{fig_performance_compare}
\end{figure}

% 2.问题：介绍RWKV的memory-bound和vast size
Despite the remarkable performance of RWKV, its vast size of parameters have posed a significant barrier to the deployment on resource-constrained devices. 
Firstly, RWKV models are heavily memory-bound during inference. 
For instance, the compute-to-memory access ratio (FLOPs/Bytes) of RWKV-6-7B~\cite{peng2024eagle} is 0.97, while that for the decoding phase of LLaMA-2-7B~\cite{touvron2023llama2} is 4.88. 
Secondly, large RWKV models demand substantial memory resources. 
For instance, RWKV-6-14B requires approximately 30GB of memory to be loaded, which typically exceeds the capacity of edge devices. 
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{imgs/heatmap.png}
    \caption{Zero-shot accuracy when applying different quantization methods to specific weights. For the weight in each sub-figure, $\mathrm{SQ}_{\mathrm{acc}}$ denotes the performance when SQ is applied, $\mathrm{VQ}_{\mathrm{acc}}$ denotes the performance when VQ is applied, while all other weights are quantized with VQ. $P_c$ and $P_f$ are coarse- and fine-grained proxy, while $\mu_c$ and $\mu_f$ are their corresponding thresholds. }
    \label{fig_proxy_methods}
\vspace{-2mm}
\end{figure*}

% 3.引入量化和融合问题
Quantization is an essential technique for deploying deep neural networks (DNNs) in environments with limited computational resources. 
Although this method has been successfully utilized in T-LLMs~\cite{yuan2024llm}, its application within the RWKV family has not been systematically analyzed or studied. 
Given that both RWKV and Transformer are sequence models to be quantized, our initial solution involves exploring techniques that have been proven effective on T-LLMs.
Among these, Scalar Quantization (SQ) is the most classic and widely applied approach. 
Recent advances in SQ can be broadly categorized into smooth-based methods~\cite{lin2023awq} and rotation-based methods~\cite{liu2024spinquant, ostquant}. 
These approaches introduce smoothing vectors or orthogonal matrices to mitigate the impact of outliers. 
To avoid online computation, they typically fuse the additional parameters into neighbored normalization layers and linear layers of T-LLMs. 
However, \textbf{most of such parameters can not be absorbed into weights in context of RWKV models.} 
This is because RWKV structure employs several non-linear operators along the fusion path, including token-shift, the Sigmoid function, and the exponential function, which can impede the linear fusion process. 
As a result, the substantial runtime overhead cannot be disregarded. 
For instance, applying QuaRot~\cite{ashkboos2024quarot} to RWKV-7 series models increases the overall FLOP by more than 99\%.  

% VQ

\begin{table}[!b]
\vspace{-4mm}
\caption{The average relative clustering loss of weights for the RWKV family and the LLaMA family, computed using KMeans~\cite{lloyd1982least}. }
\vspace{-3mm}
\vskip 0.15in
\centering
\begin{tabular}{cccc}
\toprule
Family & Model & 8 Clusters & 16 Clusters \\ \midrule
\multirow{2}{*}{RWKV} & 6-7B & 2.01 & 0.78 \\
     & 6-14B & 1.98 & 0.78 \\ \midrule
\multirow{2}{*}{LLaMA} & 2-7B & 0.96 & 0.65 \\
     & 2-14B & 0.89 & 0.64 \\ \bottomrule
\end{tabular}
\label{tab_kmeans_loss}
\end{table}
In the pursuit of efficient quantization for RWKV, we identify Vector Quantization (VQ) as a highly potential approach. 
This method does not require additional online operations for the de-quantization process, yet it can effectively capture local distributions, including outliers.
For instance, quantizing LLAMA2-7B to 2 bits with VPTQ~\cite{liu2024vptq} maintains 95\% of the zero-shot performance. 
Nevertheless, \textbf{directly applying this method to RWKV models leads to significant accuracy degradation}, e.g. more than 16\% on RWKV-6-7B even at 3 bits. 
Since such cluster-based methods benefit from distinct categorical separations, RWKV models tend to have more uniform weights compared to T-LLMs, thereby posing challenges for the clustering process as shown in Table~\ref{tab_kmeans_loss}. 
Instead, we observe that directly applying classic SQ methods like GPTQ~\cite{frantar2022gptq} to them can enhance the performance as shown in Figure~\ref{fig_proxy_methods}(c). 
This finding indicates a promising solution by selecting between SQ and VQ in consideration of different distributions of weights. 

% 我们的方法
To this end, we propose RWKVQuant, an effective and efficient post-training quantization (PTQ) framework tailored for RWKV models. 
Our core insight is to identify an optimal hybrid strategy that maximizes the respective strengths of SQ and VQ, thereby enhancing their individual performance as illustrated in Figure~\ref{fig_performance_compare}. Specifically, we propose a multi-scale proxy to guide each weight. 
(1) The coarse-grained proxy is established on the basis of Information Entropy (IE)~\cite{shannon1948mathematical}, which evaluate the overall uniformity. For non-uniform weights, VQ is directly applied as shown in Figure~\ref{fig_proxy_methods}(a). 
(2) For uniform weights, we further introduce a fine-grained proxy, computed by weighted hight-order central moments, to detect local outliers. VQ is applied when outliers emerge, as shown in Figure~\ref{fig_proxy_methods}(b); otherwise, SQ is applied as shown in Figure~\ref{fig_proxy_methods}(c). 
In addition to the hybrid, we further optimize VQ for the unique element-wise multiplication operator of RWKV. 
Lastly, our contributions can be concluded as follows. 
\begin{itemize}
    \item We identify that advanced PTQ frameworks, i.e., smooth-based and rotation-based SQ methods, are not well-suitable for RWKV primarily due to the unavoidable runtime overhead. 
    Further, our analysis reveals that the hybrid of VQ and classic SQ methods can efficiently achieve superior performance.
    \item We propose RWKVQuant. 
    We introduce a multi-scale proxy to guide the hybrid strategy. 
    And we further enhance the VQ for the unique element-wise multiplication modules in RWKV.
    \item RWKVQuant can effectively quantize weights into about 3-bit and outperforms both SQ and VQ methods, e.g., less than 1\% zero-shot accuracy drop on RWKV-6-14B. 
    \item To the best of our knowledge, RWKVQuant is the first comprehensive PTQ framework for the RWKV family. 
    As a pioneering study, we will publish the \textcolor{red}{\href{https://anonymous.4open.science/r/RWKVQuant-5B27/README.md}{code}} in the hope of promoting further research and facilitating advancements in this field.
\end{itemize}


==> texs/2_related_work.tex <==
\section{Related Work}\label{sec_related_work}

\subsection{RWKV Family}\label{subsec_rwkv_works}
RWKV~\cite{peng2023rwkv, peng2024eagle} models employ a distinctive key-value methodology to sequentially handle dependencies.
Compared to Transformers~\cite{vaswani2017attention}, this technique substantially decreases the computational overhead and memory demands while effectively retaining the capacity to model long-term dependencies. 
The RWKV family has already manifested its potential in a diverse array of applications~\cite{li2024survey}. 
For Natural Language Processing (NLP) tasks, RWKV has been effectively utilized in producing web novels~\cite{peng-ai-writer}. 
It also serves the chatbot projects of QQ~\cite{qq}, WeChat~\cite{wechat1, wechat2}, and Telegram~\cite{telegram}. 
In the realm of Natural Language Understanding (NLU) tasks, RWKV-v6~\cite{peng2024eagle} has achieved remarkable advancements in accuracy, attaining comparable performance to those of larger models like SomlLM and Qwen~\cite{chen2024onlysportslm}.
For Vision tasks, BSBP-RWKV~\cite{zhou2024bsbp} excels in the domain of medical image segmentation. 
It integrates conventional noise reduction methods with a resilient network architecture, thereby attaining superior accuracy and performance. 
In a similar vein, Restore-RWKV~\cite{yang2024restore} stands out in the restoration of medical images. 
% It incorporates a novel all-directional token translation layer and a reconstructive attention mechanism, effectively capturing the spatial correlations within 2D imagery. 

Despite the remarkable performance of RWKV, its vast size of parameters have posed a significant barrier to the deployment on resource-constrained devices. 
Firstly, RWKV models are heavily memory-bound during inference. 
For instance, the compute-to-memory access ratio (FLOPs/Bytes) of RWKV-6-7B~\cite{peng2024eagle} is 0.97, while that for the decoding phase of LLaMA-2-7B~\cite{touvron2023llama2} is 4.88. 
Secondly, large RWKV models demand substantial memory resources. 
For instance, RWKV-6-14B requires approximately 30GB of memory to be loaded, which typically exceeds the capacity of edge devices. 

\subsection{Quantization Methods}\label{subsec_ptq_works}
Quantization serves as a potent strategy for model compression. It can be divided into two main approaches: Quantization Aware Training (QAT) and Post Training Quantization (PTQ). QAT often requires training with complete parameters, which can be impractical for large-scale models. In contrast, PTQ has become a focal point for research. By converting the high-precision variables of pre-trained models into low-bit integers, PTQ achieves a reduction in memory usage and an acceleration of inference speed. 
Generally, recently advanced PTQ frameworks can be divided into two types: SQ and VQ. 

\paragraph{Scalar quantization (SQ)} 
SQ is widely-adopted by most of the PTQ frameworks. It maps the original data to the quantized range by a scaling factor, and subsequently rounds floating points to the uniform-distributed integers. 
For instance, GPTQ~\cite{frantar2022gptq} quantizes weights to 3-4 bit with slight accuracy drop based on approximate second-order information. 
AWQ~\cite{lin2023awq}, SmoothQuant~\cite{xiao2022smoothquant}, and OmniQuant~\cite{2023omniquant} explore the scheme of smoothing by detecting the importance of different activation channels. 
Recent works (e.g., Quarot~\cite{ashkboos2024quarot}, SpinQuant~\cite{liu2024spinquant}, and OSTQuant~\cite{ostquant}) further suppress outliers by utilizing computation-invariant rotation transformation. The typically multiply the variables that to be quantized with an orthogonal matrix. 
Both smoothing and rotation are intended to make the original distribution more uniform, thus reducing the rounding error of SQ.

\paragraph{Vector quantization (VQ)} 
VQ has recently gained a lot research attention for its higher accuracy in lower bit settings. It first reshapes the original tensor into vectors, then maps them to a finite subset, which is commonly referred to as a codebook. Compared to SQ, this scheme takes the advantage of maintaining the shape of the source distribution.
For example, VPTQ~\cite{liu2024vptq} and GPTVQ~\cite{van2024gptvq} combine VQ with GPTQ, achieving advanced performances under 2$\sim$3 bits. To obtain the codebook, they cluster the source vectors by K-Means Algorithm~\cite{lloyd1982least} and Expectation-Maximization Algorithm~\cite{moon1996EM}, respectively. AQLM~\cite{egiazarian2024extreme} further utilize layer-wise training for the codebook to get optimal accuracy. 
These methods essentially represent the original data source in the form of clustering.
% 有个疑问，quip，quip#,pvq之类的是把源分布做均匀，跟本文的主旨不符，还要不要提 

% 建议简单提一下。但不过多claim。

% K-means溯源一下增加一下citation？


% While both SQ and VQ perform effectively for Transformer-based large language models, they do not work well with RWKV models. 
% 要不要说这一句↓ 
% 这一句可以酌情放到Intorduction里.related work里放在此处，一般情况下reviewer看不太到.
% Notably, to our knowledge, our method is the first PTQ solution specifically designed for the RWKV family, applicable to both RWKV-based language and vision tasks.



